PixInWav: Residual Steganography for Hiding Pixels in Audio

Steganography comprises the mechanics of hiding data in a host media that may be publicly available. While previous works focused on unimodal setups (e.g., hiding images in images, or hiding audio in audio), PixInWav targets the multimodal case of hiding images in audio. To this end, we propose a novel residual architecture operating on top of short-time discrete cosine transform (STDCT) audio spectrograms. Among our results, we find that the residual audio steganography setup we propose allows independent encoding of the hidden image from the host audio without compromising quality. Accordingly, while previous works require both host and hidden signals to hide a signal, PixInWav can encode images offline -- which can be later hidden, in a residual fashion, into any audio signal. Finally, we test our scheme in a lab setting to transmit images over airwaves from a loudspeaker to a microphone verifying our theoretical insights and obtaining promising results.

==> figures/beta-span.tex <==
\begin{figure}%[b]
\centering
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=.24\columnwidth]{figures/beta/beta_0.05_image.png}
    \includegraphics[width=.24\columnwidth]{figures/beta/beta_0.1_image.png}
    \includegraphics[width=.24\columnwidth]{figures/beta/beta_0.5_image.png}
    \includegraphics[width=.24\columnwidth]{figures/beta/beta_0.9_image.png}\\
    \includegraphics[width=.24\columnwidth]{figures/beta/beta_0.05_spec_2.png}
    \includegraphics[width=.24\columnwidth]{figures/beta/beta_0.1_spec_2.png}
    \includegraphics[width=.24\columnwidth]{figures/beta/beta_0.5_spec_2.png}
    \includegraphics[width=.24\columnwidth]{figures/beta/beta_0.9_spec_2.png}
%    \caption[short]{Res-Indep}
\end{subfigure}\\
\caption[short]{Effect of $\beta$ on the image and spectrogram. Each column refers to a $\beta = \{0.05, 0.1, 0.5, 0.9$\}, respectively.}
\label{fig:beta-span}
\end{figure}


==> figures/equalization-baboon.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{figures/onair-supplementary/equalization-baboon.png}
\caption[short]{\textbf{The effect of equalization:} the first image corresponds to the original \textit{baboon} image which was encoded in the audio spectrogram. After transforming the container spectrogram back to a waveform and transmitting it through the air by a loudspeaker and recording with a microphone, we obtain the second image. The third image is the yielded output after applying pixel-based histogram equalization to the revealed image.}
\label{fig:baboon-onair}
\end{figure}


==> figures/image_onair.tex <==
\begin{figure}[h]
\centering
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/onair-supplementary/baboon_air.png}
    \caption[short]{Original and the average of revealed and equalized images}
\end{subfigure}\\
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/onair-supplementary/baboon_channels.png}
    \caption[short]{Binarized RGB channels with threshold $=1/2$}
\end{subfigure}\\

\caption[short]{\textbf{Multiple images in transmission:} 126 images of size $256 \times 256 \times 3$ were encoded in an audio clip of duration $192$ seconds at 44,100Hz. This corresponds to an audio clip of 8,467,680 samples. Each image was encoded in a section of 67,522 samples, consecutively. }
\label{fig:image-onair}
\end{figure}


==> figures/noise-qualitative2.tex <==
\begin{figure}%[b]
\centering
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_no_noise_vd_no_noise.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_no_noise_vd_gauss_0.1.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_no_noise_vd_gauss_0.5.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_no_noise_vd_gauss_0.75.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_no_noise_vd_gauss_0.9.png}
    \caption[short]{Train: -, Test: AWGN.}
\end{subfigure}\\
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_gauss_0.1_vd_no_noise.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_gauss_0.1_vd_gauss_0.1.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_gauss_0.1_vd_gauss_0.5.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_gauss_0.1_vd_gauss_0.75.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_gauss_0.1_vd_gauss_0.9.png}
    \caption[short]{Train: AWGN, Test: AWGN.}
\end{subfigure}\\
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_speckle_0.1_vd_no_noise.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_speckle_0.1_vd_gauss_0.1.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_speckle_0.1_vd_gauss_0.5.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_speckle_0.1_vd_gauss_0.75.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_speckle_0.1_vd_gauss_0.9.png}
    \caption[short]{Train: Speckle, Test: AWGN.}
\end{subfigure}\\
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=.19\columnwidth]{figures/noise/tr_awg_speck_vd_no_noise.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/tr_awg_speck_vd_gauss_0.1.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/tr_awg_speck_vd_gauss_0.5.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/tr_awg_speck_vd_gauss_0.75.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/tr_awg_speck_vd_gauss_0.9.png}
    \caption[short]{Train: AWGN/Speckle, Test: AWGN.}
\end{subfigure}\\
% Speckle noise
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_no_noise_vd_no_noise.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_no_noise_vd_speckle_0.1.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_no_noise_vd_speckle_0.5.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_no_noise_vd_speckle_0.75.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_no_noise_vd_speckle_0.9.png}
    \caption[short]{Train: -, Test: Speckle.}
\end{subfigure}\\
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_gauss_0.1_vd_no_noise.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_gauss_0.1_vd_speckle_0.1.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_gauss_0.1_vd_speckle_0.5.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_gauss_0.1_vd_speckle_0.75.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_gauss_0.1_vd_speckle_0.9.png}
    \caption[short]{Train: AWGN, Test: Speckle.}
\end{subfigure}\\
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_speckle_0.1_vd_no_noise.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_speckle_0.1_vd_gauss_0.1.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_speckle_0.1_vd_gauss_0.5.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_speckle_0.1_vd_gauss_0.75.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/2_tr_speckle_0.1_vd_gauss_0.9.png}
    \caption[short]{Train: Speckle, Test: Speckle.}
\end{subfigure}\\
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=.19\columnwidth]{figures/noise/tr_awg_speck_vd_no_noise.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/tr_awg_speck_vd_speckle_0.1.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/tr_awg_speck_vd_speckle_0.5.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/tr_awg_speck_vd_speckle_0.75.png}
    \includegraphics[width=.19\columnwidth]{figures/noise/tr_awg_speck_vd_speckle_0.9.png}
    \caption[short]{Train: AWGN/Speckle, Test: Speckle.}
\end{subfigure}\\
%\caption[short]{\textbf{Robustness to AWGN and speckle noise:} Each column refers, respectively, to a $\sigma=\{0, 0.1, 0.5, 0.75, 0.9$\} The model trained with AWGN at rows (b) and (e) is the most robust, also under speckle noise that was never seen during training. The worst performance corresponds to the model with any noise at training time at rows (a) and (d).}
\caption[short]{\textbf{Robustness to AWGN and speckle noise:} Each column from left to right corresponds to an increasing $\sigma=$\{$0$, $0.1$, $0.5$, $0.75$, $0.9$\} 
%The model trained with AWGN and speckle noise, depicted at rows (d) and (h), is the most robust to the other configurations, which were included in the main submission.
}

% --- the norm of the added noise.}
%\caption[short]{\textbf{Robustness to AWGN and speckle noise:} Each column refers, respectively, to a $\sigma=\{0, 0.1, 0.5, 0.75, 0.9\}$. The model trained with AWGN at rows (b) and (e) is the most robust, also under speckle noise that was never seen during training. The worst performance corresponds to the model with any noise at training time at rows (a) and (d).}
\label{fig:noise-qualitative-2}
\end{figure}

%The model trained with AWGN at rows (b) and (e) is the most robust, also under speckle noise that was never seen during training. The worst performance corresponds to the model with any noise at training time at rows (a) and (d).


==> figures/studio/studio.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/studio/setup.jpg}
    \caption{\small {\textbf{On air setup}: The speaker and microphone were faced one in front of the another and 83 centimeters apart in a laboratory environment. We used a \textit{Dynaudio acoustic Professional Monitoring system - BM6A} speaker and a \textit{Sennheiser e835} microphone. The audio WAV files were both played and recorded from a laptop connected to the speaker and microphone with a \textit{PreSonus} USB mixer.
    }}
    \label{fig:studio}
\end{figure}

==> plots/beta-more.tex <==
\pgfplotsset{compat = 1.3}
\begin{center}
\begin{minipage}{0.95\linewidth}
\resizebox{\linewidth}{!}{\begin{tikzpicture}[/pgfplots/width=0.95\linewidth, /pgfplots/height=\linewidth, /pgfplots/legend pos=south east]
\begin{axis}[
     	ymin=-16, ymax=20,
        xmin=0.05, xmax=0.9,
        ylabel=Audio SNR,
        xlabel=$\beta$,
		font=\large,
        grid=both,
		grid style=dotted,
        xmode=linear,
        ytick={-10, 0, 10, 20},
		yticklabels={-10, 0, 10, 20},
        xtick={0.1, 0.25, 0.5, 0.75, 0.9},
	    xticklabels={0.1, 0.25, 0.5, 0.75, 0.9},
        enlarge x limits=0.00,
        legend style={at={(2.16,1.1)}, anchor=North, /tikz/every even column/.append style={column sep=3.6mm}},
        legend columns = -1,
        ]
        \addlegendentry{Plain-Dep}
        \addplot[smooth,mark=x,Gray] 
          coordinates{
            (0.05,-2.901)%
            (0.1,-1.732)%
            (0.25,-2.128)%
            (0.5,-2.323)%
            (0.75,-3.193)%
            (0.9,-3.109)%
        }; 
        \addlegendentry{Res-Dep}
        \addplot[smooth,mark=x,NavyBlue] 
          coordinates{
            (0.05,6.4)%
            (0.1,9.361)%
            (0.25,8.872)%
            (0.5,5.094)%
            (0.75,4.709)%
            (0.9,3.12)%
        };
        \addlegendentry{Res-Scale}
        \addplot[smooth,mark=x,BrickRed] 
          coordinates{
            (0.05,9.341)%
            %(0.1, 0)%?????
            (0.25,6.264) %
            (0.5,3.627)%
            (0.75,2.349)%
            %(0.9,0)%??????
        };
        \addlegendentry{Res-Indep}
        \addplot[smooth,mark=x,OliveGreen] 
          coordinates{
            (0.05,11.42)%
            (0.1,9.41)%
            (0.25,6.783) %
            (0.5,5.42)%
            (0.75,4.87)%
            (0.9,1.56)%
        };
    \end{axis}

\begin{axis}[
    	ymin=0.3, ymax=1.0,
        xmin=0.1, xmax=0.9,
        ylabel=image SSIM,
        xlabel=$\beta$,
		font=\large,
        grid=both,
		grid style=dotted,
        xmode=linear,
        ytick={0.90, 0.95, 1.00},
		yticklabels={0.90, 0.95, 1.00},
        xtick={0.1, 0.25, 0.5, 0.75, 0.9},
	    xticklabels={0.1, 0.25, 0.5, 0.75, 0.9},
        enlarge x limits=0.00,
        ylabel shift=0.0cm,
        xshift=8.5cm
        ]
        
        \addplot[smooth,mark=x,Gray] 
          coordinates{
            (0.05,0.7926)%
            (0.1,0.9338)%
            (0.25,0.8824)%
            (0.5,0.9448)%
            (0.75,0.9635)%
            (0.9,0.9453)%
        }; 
        \addplot[smooth,mark=x,NavyBlue] 
          coordinates{
            (0.05,0.7667)%
            (0.1,0.7838)%
            (0.25,0.8117)%
            (0.5,0.8228)%
            (0.75,0.866)%
            (0.9,0.8682)%
        };
        \addplot[smooth,mark=x,BrickRed] 
          coordinates{
            (0.05,0.4213)%
            %(0.1,0)%??????
            (0.25,0.4971) %
            (0.5,0.5114)%
            (0.75,0.4775)%
            %(0.9,0)%?????
        };
        \addplot[smooth,mark=x,OliveGreen] 
          coordinates{
            (0.05,0.668)%
            (0.1,0.7611)%
            (0.25,0.7602)%
            (0.5,0.8466)%
            (0.75,0.8711)%
            (0.9,0.8267)%
        };

    \end{axis}
\end{tikzpicture}}
\end{minipage}
\end{center}

==> plots/old-beta.tex <==
% Reference: https://tex.stackexchange.com/questions/42697/pgfplots-legends-in-multiple-y-axis-plot-overlapping

\pgfplotsset{compat = 1.3}
\begin{center}
\begin{minipage}{\linewidth}
\resizebox{\linewidth}{!}{
\begin{tikzpicture}[/pgfplots/width=0.8\linewidth, /pgfplots/height=0.8\linewidth, /pgfplots/legend pos=south west]

\pgfplotsset{
    scale only axis,
    xmin=0, xmax=1.0,
    y axis style/.style={
        yticklabel style=#1,
        ylabel style=#1,
        y axis line style=#1,
        ytick style=#1
   }
}

% Axis for the audio part
\begin{axis}[
    %title={Temperature dependence of CuSO$_4\cdot$5H$_2$O solubility},
    axis y line*=left,
    y axis style=blue!75!black,
    ymin=-16, ymax=20,
    ylabel={audio SNR (dB)},
    xlabel={$\beta$},
%    xtick={0.05,0.1,0,25,0.5,0.75,0.9,1.0},
%    ytick={0,5,10,15,20},
%    legend pos=north west,
   % ymajorgrids=false,
    %grid style=dashed,
]
\addplot[smooth,mark=x,blue] 
  coordinates{
    (0.05,5.061)
    (0.25,-3.425) 
    (0.5,-9.496)
    (0.75,-12.084)
    (0.9,-15.306)
}; \label{audioSNRnoDTW}
\addplot[smooth,mark=x,blue,dashed] 
  coordinates{
    (0.05,18,41)
    (0.1,15.72)
    (0.25,12.89) 
    (0.5,9.01)
    (0.75,7.88)
    (0.9,6.23)
}; \label{audioSNRyesDTW}
\end{axis}

\begin{axis}[
  axis y line*=right,
  axis x line=none,
  ymin=0.9, ymax=1,
  ylabel={image SSIM},
  y axis style=red!75!black
]
\addlegendimage{/pgfplots/refstyle=audioSNR}
\addlegendentry{audio}
\addplot[smooth,mark=*,red] 
  coordinates{
    (0.05,0.9283)
    (0.25,0.9477) 
    (0.5,0.9585)
    (0.75,0.9671)
    (0.9,0.9718)
}; \addlegendentry{image}
\end{axis}

\end{tikzpicture}}
\end{minipage}
\end{center}

==> tables/ablation-5epochs.tex <==
% Secret resource by Kevin McGuinness for building tables
% https://people.inf.ethz.ch/markusp/teaching/guides/guide-tables.pdf
\begin{table}[h]
%\resizebox{\linewidth}{!}
\centering
%\setlength{\arrayrulewidth}{1mm}
%\setlength{\tabcolsep}{18pt}

\begin{tabular}{@{}lccc@{}}
\toprule
                     & \multicolumn{1}{c}{Audio} & \multicolumn{2}{c}{Image}\\
Architecture        & SNR $\uparrow$ & SSIM $\uparrow$ & PSNR $\uparrow$\\
%\midrule
%Plain-Dep       &  $\checkmark$ &                 &     $3.19$    & ?                   & $0.926$       & $27.90$ \\
%Res-Dep         &  $\checkmark$ & $\checkmark$    &     $3.70$    & ?                   & $0.927$       & $27.98$\\
%Res-Scale       &               & $\checkmark$     &     $3.70$    & ?                   & $0.919$       & $27.61$\\
%Res-Indep       &               & $\checkmark$     &     $4.75$     & ?                  & $0.928$       & $28.46$\\
\midrule
Res-Scale      &    $14.66$       & $0.541$       & $19.52$\\
Plain-Dep       &     $-0.73$     & $0.971$       & $32.70$ \\
Res-Dep          &     $18.80$      & $0.919$       & $27.29$\\
Res-Indep         &    $18.33$        & $0.923$       & $27.37$\\
%Res-Scale & ? & ? & ?& ?\\
\bottomrule
\end{tabular}
\caption{\textbf{Ablation study:} Audio and image quality metrics for a fixed $\beta=0.05$ with \textit{PixInWav} and the three considered baselines. Results after 5 training epochs.}
\label{tab:ablation-2}
\end{table}


==> tables/dis-noise-gaussian.tex <==
\begin{table}
\begin{tabular}{@{}ccccc@{}}
\toprule
\multicolumn{2}{c}{}                & \multicolumn{1}{c}{Audio} & \multicolumn{2}{c}{Image}\\
  Train & $\sigma$      & SNR $\uparrow$ & SSIM $\uparrow$ & PSNR $\uparrow$\\
\midrule
 -       &     -     & $18.40$            & $0.92$      & $27.37$\\
\midrule
AWGN    & $0.001$    & $18.45$          & $0.88$      & $24.09$\\
AWGN    & $0.01$     & $18.28$             & $0.86$      & $23.80$\\
AWGN    & $0.01$     & $18.30$             & $0.44$      & $17.66$\\
\midrule
Speckle & $0.001$    & $19.37$            & $0.88$      & $23.99$\\
Speckle & $0.01$     & $18.76$            & $0.88$      & $23.69$\\
Speckle & $0.01$     & $19.02$            & $0.88$      & $24.14$\\

\bottomrule
\end{tabular}
\caption{Study of the impact of the AWGN at train and test time. Results corresponds to the Res-Indep architecture ($\beta=0.005$).}
\label{tab:noise-notintrain}
\end{table}

==> tables/distortions.tex <==
% Secret resource by Kevin McGuinness for building tables
% https://people.inf.ethz.ch/markusp/teaching/guides/guide-tables.pdf
\begin{table*}
%\resizebox{\linewidth}{!}
\centering
%\setlength{\arrayrulewidth}{1mm}
%\setlength{\tabcolsep}{18pt}

\begin{tabular}{@{}lccccccc@{}}
\toprule
                &               &               &                & \multicolumn{2}{c}{Audio} & \multicolumn{2}{c}{Image}\\
Architecture    &  Conditioned  & Residual      &   DTW          & SNR $\uparrow$ & MAE $\downarrow$ & SSIM $\uparrow$ & PSNR $\uparrow$\\
\midrule
Plain-Dep       &  $\checkmark$ &               &               &     $3.19$    & ?                   & $0.93$       & $27.90$ \\
Res-Dep         &  $\checkmark$ & $\checkmark$  &               &     $3.70$    & ?                   & $0.93$     & $27.98$\\
Res-Indep       &               & $\checkmark$  &               &     $4.75$     & ?                     & $0.92$      & $27.61$\\
\midrule
Plain-Dep       &  $\checkmark$ &               &  $\checkmark$ &     $18.38$    & ?                   & $0.91$       & $26.55$ \\
Res-Dep         &  $\checkmark$ & $\checkmark$  &  $\checkmark$ &     $17.95$    & ?                   & $0.92$     & $27.53$\\
Res-Indep       &               & $\checkmark$  & $\checkmark$  & $18.40$     & ?                     & $0.92$      & $27.37$\\
%Res-Scale & ? & ? & ?& ?\\
\bottomrule
\end{tabular}
\caption{Ablation study ($\beta=0.005$).}
\label{tab:ablation}
\end{table*}

==> tables/noise-train-notatval2.tex <==
\begin{table}[h]
\begin{tabular}{@{}ccccc@{}}
\toprule
\multicolumn{1}{c}{}                & \multicolumn{1}{c}{Audio} & \multicolumn{2}{c}{Image}\\
  Noise  & SNR $\uparrow$ & SSIM $\uparrow$ & PSNR $\uparrow$\\
\midrule
 -        & $18.41$            & $0.92$      & $27.37$\\
%\midrule
%AWGN    & $0.001$    & $18.45$          & $0.88$      & $24.09$\\
%AWGN    & $0.01$     & $18.28$             & $0.86$      & $23.80$\\
AWGN $\sigma=0.1$   & $18.80$             & $0.86$      & $27.30$\\

%Speckle & $0.001$    & $19.37$            & $0.88$      & $23.99$\\
%Speckle & $0.01$     & $18.76$            & $0.88$      & $23.69$\\
Speckle $\sigma=0.1$  & $15.56$            & $0.92$      & $27.96$\\
\midrule
AWGN/Speckle & $18.80$    & $0.86$      & $27.30$ \\
\bottomrule
\end{tabular}
\caption{\textbf{Extended study of the impact of adding synthetic noise at training time in noise-free test environments:} We add a $4^{th}$ row to the results included in the main paper, that correspond to a model trained with both AWGN and speckle noises with different $\sigma=$\{$0.1$ $0.01$ $0.001$\}.
%In this case, the drop of audio SNR performance we observed when trained with speckle noise ($3^{rd}$ row) does not appear.
}
\label{tab:noise-notatval-2}
\end{table}

==> tables/sup-noise-notintrain.tex <==
\begin{table}
\begin{tabular}{@{}ccccc@{}}
\toprule
\multicolumn{2}{c}{}                & \multicolumn{1}{c}{Audio} & \multicolumn{2}{c}{Image}\\
  Noise & $\sigma$      & SNR $\uparrow$ & SSIM $\uparrow$ & PSNR $\uparrow$\\
\midrule
 -       &     -     & $18.40$            & $0.92$      & $27.37$\\
\midrule
AWGN    & $0.001$    & $18.45$          & $0.88$      & $24.09$\\
AWGN    & $0.01$     & $18.28$             & $0.86$      & $23.80$\\
AWGN    & $0.01$     & $18.30$             & $0.44$      & $17.66$\\
\midrule
Speckle & $0.001$    & $19.37$            & $0.88$      & $23.99$\\
Speckle & $0.01$     & $18.76$            & $0.88$      & $23.69$\\
Speckle & $0.01$     & $19.02$            & $0.88$      & $24.14$\\

\bottomrule
\end{tabular}
\caption{Study of the impact of the AWGN and Speckle noises over a clean stego-signal. Results corresponds to the Res-Indep architecture with $\beta=0.005$.}
\label{tab:noise-notintrain}
\end{table}
